Comparing Correspondences: Video Prediction with Correspondence-wise Losses

Image prediction methods often struggle on tasks that require changing the positions of objects, such as video prediction, producing blurry images that average over the many positions that objects might occupy. In this paper, we propose a simple change to existing image similarity metrics that makes them more robust to positional errors: we match the images using optical flow, then measure the visual similarity of corresponding pixels. This change leads to crisper and more perceptually accurate predictions, and does not require modifications to the image prediction network. We apply our method to a variety of video prediction tasks, where it obtains strong performance with simple network architectures, and to the closely related task of video interpolation. Code and results are available at our webpage: https://dangeng.github.io/CorrWiseLosses

==> sections/1_intro.tex <==
\section{Introduction}


Recent years have seen major advances in image prediction methods~\cite{isola2016pix2pix, chen2017CRN, park2019spade, karras2018stylegan, brock2018biggan}, yet the situations where they can be used remain stubbornly limited. Today's methods can successfully alter a scene's texture, color, or lighting, but struggle to make even tiny changes to {\em position}.  Due to these limitations, video prediction remains a challenging open problem. The fundamental uncertainty of predicting where, exactly, an object will be in the future leads off-the-shelf image synthesis methods to produce blurry, hedged images that average over all possible positions.

One successful line of work has addressed this problem with {\it flow-based} architectures. These architectures ``copy and paste'' existing image content into a prediction, typically by predicting an optical flow field and using it to warp the input video frames~\cite{zhou2016flow,liu2017video,gao2019disentangling,jaderberg2015spatial}. Since by construction every pixel in the predicted image has a correspondence in a previous frame, the resulting images are unlikely to be blurry. These methods, however, require complex network designs, with special layers for motion prediction and warping, making it challenging to integrate them with traditional image synthesis models. They also require other prediction mechanisms to handle image content that cannot be generated via warping (e.g. occlusions).


Architectures that directly synthesize pixels, by contrast, are simpler and more general. 
We argue that their poor performance is a direct result of the loss function, and we propose a simple change to existing losses that makes them more robust to small positional errors. When comparing two images, we put them into correspondence using optical flow, then measure the similarity between {\em matching pairs of pixels}. Comparisons between the images therefore occur between pixel correspondences, rather than pixels that reside in the same spatial positions (\fig{fig:teaser}), i.e., the loss is computed {\it correspondence-wise} rather than pixel-wise.

Despite its simplicity, our proposed ``loss extension" leads to crisper and more accurate video predictions. To obtain low loss, the predicted images must be ``easy to match" with the ground truth via optical flow: every pixel in a ground truth image requires a high-quality match in the predicted image, and vice versa.

Blurry predictions tend to obtain high loss, since there is no simple, smooth flow field that puts them into correspondence with the ground truth. The loss also encourages objects to be placed in their {\em correct} positions: positional mistakes lead to poor quality matches and missing content, both of which incur large penalties.

Crucially, our method is {\em architecture-agnostic}, and we show strong performance with a simple, off-the-shelf image prediction network. In contrast to flow-based networks our approach can account for events that cannot be synthesized by copying and pasting pixels, such as disocclusions or lighting changes, and because of our loss our network produces crisp images.

We apply our method to the task of predicting future frames of egocentric driving videos. We demonstrate its effectiveness a variety of ways. First, we show through ablation experiments on next-frame prediction that our method improves image quality of existing similarity metrics, such as $L_1$ distance and perceptual losses~\cite{gatys2016image,johnson2016perceptual}. Second, we apply our method to multi-frame video prediction. Despite using a simple off-the-shelf image-translation architecture and a perceptual loss, we obtain results that outperform a flow-based state-of-the-art method~\cite{wu2020future} on perceptual quality metrics for KITTI~\cite{geiger2013IJRR} and Cityscapes~\cite{Cordts2016Cityscapes} videos. Finally, we show that our method can be used to improve stochastic, variational autoencoder-based  methods~\cite{denton2018stochastic,villegas2019high}.



==> sections/1_intro_general.tex <==
\section{Introduction}

Pixelwise losses, such as L1 or MSE losses, are simple yet pervasive in computer vision, and are surprisingly effective. They are used as the only loss in many prominent models~\cite{}, and are a component of the loss in the vast majority of methods~\cite{}. The simplicity of pixelwise losses comes from the fact that they are defined by the assumption that pixels should be compared based only on their location in an image.

This assumption makes pixelwise losses incredibly easy to implement and highly effective, but can also cause problems. For example, when used for image generation or video prediction, it is well known that this class of losses creates images that are blurry. Generated images ``hedge" over uncertainty in the location of objects. Rather than committing to a single location, models trained with pixelwise losses choose an expectation of all possible locations simultaneously. 

When faced with problems  that pixelwise losses performed poorly on, such as template matching, early practitioners of computer vision developed methods that were less sensitive to the absolute location of objects such as the Hausdorff or Chamfer distances. However, in recent years these ideas seem to have been largely forgotten. In this paper, we shed a modern light on these classical ideas, and present an extension to pixelwise losses in the spirit of these metrics.

Our key idea is to compare pixels not by location, but by their {\it visual correspondences}. By using this idea for image generation, models no longer benefit from ``hedging" predictions. They are instead incentivized to first produce high quality ``matchable" images and then move objects closer to their ground truth location in order to minimize the distance between correspondences, reducing blurriness and improving robustness under high uncertainty. 

In order to find visual correspondences, we propose to use an off-the-shelf optical flow network. These models provide dense pixel-level correspondences, are fully differentiable, and provide a certain amount of ``inductive bias" to the loss...

We will show how to use optical flow to find dense pixel correspondences, and present an efficient way to calculate a correspondence-wise loss. We find that using the resulting loss in various image generation tasks results in robustness to high spatial uncertainty, predictions that do not suffer from hedging, and crisper and more accurate generated images. 

While blurry images may result in a low pixelwise loss due to hedging, a correspondence-wise loss implicitly enforces sharpness because blurry images are harder to match to the ground truth via optical flow: every pixel in a ground truth image requires a high-quality match in the predicted image, and vice versa. The loss also encourages objects to be placed in their {\em correct} positions: positional mistakes lead to poor quality matches and missing content, both of which incur large penalties.

This formulation can also naturally incorporate losses that operate on the positions of the corresponding pixels. This includes losses that penalize complex, long-range matches, such as by penalizing the distance between matches or the magnitude of the flow field gradients. The resulting loss resembles the energy functional of classic Horn and Schunck-style~\cite{} optical flow methods and can naturally be extended to use recent edge-aware losses.

We demonstrate the effectiveness of our method on future video prediction, frame interpolation, and model predictive control. In video prediction we achieve results competitive with state-of-the-art. We extensively ablate the corrwise loss with pixelwise counterparts on a variety of settings and datasets and show that using our loss produces higher quality images as judged by quantitative metrics and human studies. In frame interpolation we show that replacing the loss of an off-the-shelf method~\cite{kalluri2020flavr} improves the accuracy and quality of its image predictions. And finally, we show that our loss can offer benefits over traditional costs in model predictive control.



==> sections/old.tex <==
%, without committing to any single one.


% %What makes these tasks different is the highly multimodal nature of the prediction problem. Simple ``pixelwise" losses, such as per-pixel $L_2$ distance, assign large penalties to even tiny errors in structure. 
% Predicting an object's position incorrectly under such a loss is can be a catastrophic error, and consequently image synthesis models avoid this situation by hedging --- creating blurry images that average over the many possible positions an object might be, without committing to any single one.

%, creating blurry images.

%that an object is in one position, when really it is in another, can be a catastrophic error. 

%in structure; predicting an object's position incorrectly is a catastrophic error. Consequently, models 
%predicting that an object is in one location, when it really is in another, is treated as a catastrophic error. Consequently, 

%not always correlated with the magnitude of the positional error; a few pixels of positional error will often incur the same penalty as a large shift. Due to these issues, a model trained to optimize a pixelwise loss will hedge its predictions over the many possible object positions, creating blurry results. 
%(\fig{fig:cow_reconstruction}). % some people don't like fig 2 references to become fig 1 for some reason


%This strong constraint provides the model with a degree of robustness to positional errors. 

%Errors in position still contribute significantly to the loss, however, since 

% but---crucially---it is not invariant to predicted object positions. The ground truth image is still the global minimum, and positioning errors contribute significantly to the loss, since they reduce the quality of the correspondences in the ground truth image. Moreover, blurry ``hedged" predictions obtain higher loss than predictions that commit to a single, coherent prediction that contain a pool of correspondences. 

% The errors 
%The global minimum of the loss remains the same (i.e. the ground truth image itself).  

%but it also encourages images that contain a single correct prediction instead of blurry hedged results. 


% properties of our method:
% - if the image content doesn't have a correspondence, then you pay a price (occlusions)
% - "global minimum" are same between base loss and our method
% - much more likely to get the correspondence correct if you put it in the right position 
% - if your predicted image is matchable, then you pay a low cost. if it's hard to match you pay a high cost. how matchable is your predicted image with the ground truth?
% - flow algorithms want smooth flow



%For example, ... generates a future frame of a video by predicting an optical flow field, and then resampling the input to match it. 

%The other major approach is to add an explicit representation of motion inside an architecture. For example, 

%has been to add an explicit representation of motion as an inductive bias inside a predictor. 

% approach is to explicitly model motion inside the architecture. 

% to cover them all without hedging over some modes.

%However, this often makes the problem harder, not easier, as the number of modes can be extremely large. 
%the number of possible modes can be quite large, making it challenging to train a model that covers the full distribution without at least partially blurring over multiple modes. 

%Other research uses perceptual losses derived from image features~\cite{gatys2016image, dosovitskiy2016generating, johnson2016perceptual, chen2017CRN} to exploit the invariances learned by object recognition models, or by human studies~\cite{zhang2018lpips}. While these losses work well when the misalignments between the prediction and ground truth are small, they fail for large misalignments. 


%In this paper, we take inspiration from classic deformable image matching methods, such as Chamfer distance~\cite{barrow1977parametric,huttenlocher1993comparing} that explicitly account for geometric misalignment. 


%Instead of simple change to off-the-shelf loss functions that first puts the pixels in the two images into correspondence, and then compare the similarity of corresponding pixels. 

%We propose a simple extension of existing loss functions that

%We propose a simple extension of image similarity functions. 

%We propose to make a simple change to off-the-shelf loss functions

% make a simple change to an off-the-shelf loss function

%and deformable parts models~\cite{fischler1973representation,felzenszwalb2005pictorial,felzenszwalb2009object}, that explicitly model the geometric misalignment between two images when assessing their similarity. 

%We propose {\em \methodName},  a simple modification to existing similarity metrics: prior to computing an off-the-shelf  similarity metric, we warp the image to match its target using an estimated optical flow. Similarity is then measured between the warped image and ground truth image. Despite the simplicity of this approach, we show that it has a number of desirable properties that make it well-suited to image prediction tasks (\fig{fig:toy_problem}). %% It is invariant to the global positions of scene structures, but is still sensitive to their {\em relative} positions;
%The ground truth solution has zero loss, but errors in positioning result in approximately proportionate increases in the loss;  it discourages the blurred solutions often favored by simple pixelwise losses when there is positional uncertainty; and it is efficient to compute without the need for stochasticity.


% needs better motivation and name
%In this paper, we take inspiration from classic image matching methods, such as Chamfer distance~\cite{barrow1977parametric,huttenlocher1993comparing} and deformable parts models~\cite{fischler1973representation,felzenszwalb2005pictorial,felzenszwalb2009object}, that explicitly model the geometric misalignment between two images when assessing their similarity. We propose {\em \methodName},  a simple modification to existing similarity metrics: prior to computing an off-the-shelf  similarity metric, we warp the image to match its target using an estimated optical flow. Similarity is then measured between the warped image and ground truth image. Despite the simplicity of this approach, we show that it has a number of desirable properties that make it well-suited to image prediction tasks (\fig{fig:toy_problem}). %% It is invariant to the global positions of scene structures, but is still sensitive to their {\em relative} positions;
%The ground truth solution has zero loss, but errors in positioning result in approximately proportionate increases in the loss;  it discourages the blurred solutions often favored by simple pixelwise losses when there is positional uncertainty; and it is efficient to compute without the need for stochasticity.





%% We apply our loss to the task of predicting future frames of a video. We demonstrate the effectiveness of our loss in a variety of ways: 1) We show that we predict future frames of first-person driving videos from the KITTI~\cite{geiger2013IJRR} and KTH datasets. The resulting predictions are rated as significantly more plausible by human observers on a ``real vs. fake'' psychophysical study. We also obtain higher accuracy on quantitative metrics that measure the accuracy of the locations of objects in a scene. 2) We verify that the loss measured by our model more closely matches human perceptions 3) We adapt our loss to video prediction. Despite our loss's simplicity, we obtain videos that are rated as significantly more plausible than those of state-of-the-art video future prediction methods.


%~\cite{geiger2013IJRR} and human actions~\cite{}




%Could a ``lazy" prediction model, for instance, place objects in incorrect locations, and incur zero loss when optical flow corrects its mistake? 

%We extend the example in~\fig{} so that the object's 2D position is sampled uniformly at random in a square centered on the image center. 
%if we predict that the object is in one position, when it is really in another, we show the loss that we incur. 
%In~\fig{fig:toy_problem}, we plot the behavior of the $ L_1 $ metric and \methodName as a function of predicted object location.
%where the ground truth image is exactly in the center of the image. Doing so we obtain the contour plots in~\fig{fig:cow_contours}: 
%The plots show the error incurred for predicting the object at a given location, when its true location is at the image center. For this, we averaged the loss over a dataset of images (see supp. material for details).
%Given that our method ``snaps" objects into place, one may expect our loss function to have a large basin of low loss and a correspondingly poor gradient signal.  % AO: not sure I understand the gradient signal part


%We ask how the loss behaves on image prediction tasks in which there is inherent uncertainty in object position. 
%We compute the average image under our similarity metric, $\loss_{sym}$, with base loss $\loss = L_1$. We visualize the average image under the $L_1$ loss and under $\mathcal{L}_{warp}$ with a base loss of $ \mathcal{L} = L_1$. 
%This is the image that a model should, under ideal conditions, predict given the uncertainty in the object position. It is found by searching for the image $\bar{\im}$ that minimizes $\Ex_{\im \in \mathcal{D}}[\mathcal{L}(\bar{\im}, \im)]$, where $\mathcal{D}$ is the collection of images and $\mathcal{L}$ is the loss. The resulting average under the $L_1$ loss (corresponding to the median) is very blurry (\fig{fig:toy_problem}b). This result is similar for other pixelwise losses, such as $L_2$, which is significantly blurrier (see supp. material).
%for the average image under the $ L_1 $ distance metric (known empirically to produce sharper images than $L_2$~\cite{isola2016pix2pix}), i.e. finding an image $\hat{\im}$ that minimizes $\Ex[]$ results in an blurry reconstruction. %Evidently, the $ L_1 $ metric seems to believe that these images are significantly different. 
%In contrast, optimizing for \methodName, with an $ \mathcal{L} = L_1 $ base loss,%

%The resulting image average image produces a crisp image, with the object approximately at the center, $\frac{1}{2}(x_1 - x_0)$. By contrast, the average image from $L_1$ loss alone (i.e. the median) and perceptual loss~\cite{johnson2016perceptual} are blurry images that superimpose the object in every timestep. In all cases, we estimate an image $\imest$ that minimizes $\Ex_{\im \in \mathcal{D}}[\loss_C(\bar{\im}, \im)]$ using stochastic gradient descent, where $\mathcal{D}$ is the set of video frames \supparxiv{(see supplementary for details)}{(see \sect{} for details)}.

%Since the blurry image cannot be matched easily to the ground truth. Conversely, our sharp reconstructions actually attain a higher $ L_1 $ loss, despite looking perceptually better than the median image. In the supplementary material, we show that these results holds for a wide range of different perturbations, objects, and backgrounds.


%An object in the first frame with $x$-coordinate $x_0$ moves horizontally with an unknown velocity, such that its new position is uniformly distributed in $[x_0, x_1]$. 

%We sample a collection of images with a static background and a single object composited inside. Its location is subtly different between images, sampled uniformly at random from within a small centered window. These images are often indistinguishable without close examination, as shown in~\fig{fig:toy_problem}a.   


% \mypar{A simple prediction task.}  We ask how a model trained to estimate an image will behave when there is inherent uncertainty in object position (\fig{fig:toy_problem}). We sample a collection of images with a static background and a single object composited inside. Its location is subtly different between images, sampled uniformly at random from within a small centered window. These images are often indistinguishable without close examination, as shown in~\fig{fig:toy_problem}a.   

%We ask how different loss functions reconstruct this collection of images, and measure 

%\mypar{Image Averages} 
%We visualize the average image under the $L_1$ loss and under $\mathcal{L}_{warp}$ with a base loss of $ \mathcal{L} = L_1$. 
%This is the image that a model should, under ideal conditions, predict given the uncertainty in the object position. It is found by searching for the image $\bar{\im}$ that minimizes $\Ex_{\im \in \mathcal{D}}[\mathcal{L}(\bar{\im}, \im)]$, where $\mathcal{D}$ is the collection of images and $\mathcal{L}$ is the loss. The resulting average under the $L_1$ loss (corresponding to the median) is very blurry (\fig{fig:toy_problem}b). This result is similar for other pixelwise losses, such as $L_2$, which is significantly blurrier (see supp. material).
%for the average image under the $ L_1 $ distance metric (known empirically to produce sharper images than $L_2$~\cite{isola2016pix2pix}), i.e. finding an image $\hat{\im}$ that minimizes $\Ex[]$ results in an blurry reconstruction. %Evidently, the $ L_1 $ metric seems to believe that these images are significantly different. 
%In contrast, optimizing for \methodName, with an $ \mathcal{L} = L_1 $ base loss,%

%In contrast, our loss obtains a sharp reconstruction that retains almost all of the object detail. 
%Under our loss, blurry images attain significantly higher loss than crisp ones, since the blurry image cannot be matched easily to the ground truth. Conversely, our sharp reconstructions actually attain a higher $ L_1 $ loss, despite looking perceptually better than the median image. In the supplementary material, we show that these results holds for a wide range of different perturbations, objects, and backgrounds.

% \mypar{Loss Landscape} Next, we ask how the loss changes as a function of positional error. %if we predict that the object is in one position, when it is really in another, we show the loss that we incur. 
% In~\fig{fig:toy_problem}c, we plot the behavior of the $ L_1 $ metric and \methodName as a function of predicted object location.
% %where the ground truth image is exactly in the center of the image. Doing so we obtain the contour plots in~\fig{fig:cow_contours}: 
% The plots show the error incurred for predicting the object at a given location, when its true location is at the image center. For this, we averaged the loss over a dataset of images (see supp. material for details).
% %Given that our method ``snaps" objects into place, one may expect our loss function to have a large basin of low loss and a correspondingly poor gradient signal.  % AO: not sure I understand the gradient signal part




%Errors in the flow prediction %, especially for large object shifts,  %AO: not sure I get this
%result in a gradually increasing loss. 

 %We see that \methodName has a smoothly varying loss surface, with a minima at the ground truth position. By contrast, $L_1$ is less smooth, and it depends significantly on the object shape and its appearance. For example, since the object (shown in~\fig{fig:toy_problem}a) was wider than it was tall, vertical positioning errors incur significantly higher loss than horizontal ones; the former lead to errors in pixels across the (larger) top/bottom sides of the object, the latter to errors along the (smaller) left/right sides. Additionally, local minima appear on both sides of center, probably as a result of the object's texture.


%Given that our method partially ``snaps" objects into place, one may ask whether our loss function is {\em invariant} to tiny errors in position, \eg with a basin of near-zero loss near the object position. However, we can see that this is not the case; the loss increases smoothly with distance. Images with errors in object position lead to commensurately larger \methodName. This is both because an erroneous prediction will often be missing image content, such as occluded or disoccluded regions, and because optical flow methods explicitly trade-off between image reconstruction (Eq.~\ref{eq:warpdist}) and smoothness of the underlying flow (please see the supp. material for more discussion). This property allows \methodName to better place objects within generated images, as can be seen in our experiments as well as in~\fig{fig:teaser}.

% For example, we can see in~\eqn{eq:}

%The errors in the images after warping have many source

% Assuming a Horn-Schunck-style optical flow, our loss can be written as:
% %% \begin{eqnarray}
% %%   \mathcal{L}_{F}(I, \hat{I}) &=& \norm{I - \warp(I, \flowfn(I, \hat{I}))}_1 \\
% %%  &=& \norm{I - \warp(I, \left[\argmin_F \norm{I - \warp(I, F)} + \norm{\nabla F} \right]) }_1 \\
% %% \end{eqnarray}
% \begin{eqnarray}
%   %  \mathcal{L}_{F}(I, \hat{I}) = \norm{I - \warp(I, \flowfn(I, \hat{I}))}_1 \\
%   \mathcal{L}_{F} &=& \\
% &   =& \norm{I - \warp(I, \flowfn(I, \hat{I}))}_1 \\
% &  =& \norm{I - \warp(I, \argmin_F [\norm{I - \warp(I, F)} + \norm{\nabla F} ]) }_1 \\
% \end{eqnarray}


% %% First, we see that $\mathcal{L}_{F}(\im, \imest)$ is a lower bound on
% %% $\norm{\nabla \flowfn}$, since it's equal to the photoconsistency term
% %% from the optical flow after warping.

% Writing the loss this way suggests that there is a trade-off between
% reconstruction accuracy, $\norm{I - \warp(I, F)}$ and flow
%   smoothess. This trade-off will cause incorrectly positioned objects
%   to incur larger recontruction losses. Perfect reconstruction becomes
%   increasingly expensive for the flow model, so it chooses a solution
%   with higher reconstruction loss.
  
  
%In contrast to the $ L_1 $ plots, our loss avoids a sharp minima and provides a smooth error signal that %good gradient signal over a large range of object positions. We attribute the success of \methodName in the later experiments in part to this fact.


% One of our goals is to reduce the {\em blurring} that occurs in image prediction tasks when there is uncertainty in object positions. To help understand why this behavior happens, and how \methodName addresses it, consider the toy image prediction task shown in~\fig{fig:toy_data}. %~\andrew{Consider using the Flying Chairs dataset instead}. 

% We sample a dataset of images with a static background and a single object composited in. The location of this object is different between images, but is imperceptibly so. To a human, the images in the dataset are almost indistinguishable as shown in~\fig{fig:toy_data}. Despite this, a model trained to find the average image under the $ L_1 $ distance metric (known empirically to produce sharper images~\cite{isola2016pix2pix}) results in an incredibly blurry reconstruction (note that this should be the median of the dataset). Evidently, the $ L_1 $ metric seems to believe that these images are significantly different. In contrast, optimizing for our \methodName, with an $ L_1 $ base loss, we find that the reconstruction is sharp and retains almost all of the object detail. Our similarity metric is able to ignore the pixel shifts that confused the $ L_1 $ metric, and corresponds better to human perception. In the supplementary material, we show that this result holds for a wide range of different perturbations, objects, and backgrounds.

% In addition to calculating image averages, we can also plot the behavior of the $ L_1 $ metric and \methodName as a function of object location, with the target image being the object in exactly the center of the image. Doing so we obtain the contour plots in~\fig{fig:cow_contours}. Given that our method ``snaps" objects into place, one may expect our loss function to have a large basin of low loss and a correspondingly poor gradient signal. This is however not the case. Errors in the flow prediction, especially for large object shifts, result in a more gradual loss landscape. In contrast to the $ L_1 $ contour plots our loss avoids a sharp minima and provides good gradient signal over a large range of object positions. We attribute the success of \methodName in the later experiments in part to this fact.

% \subsection{Implementation Details}\label{sect:implementation}
% \vspace{3mm}

% \mypar{Avoiding Local Minima} We found that the loss can be susceptible to falling into local minima during, especially during the early stages of training when (artifact-heavy) images obtain very long-range correspondences. To address this, we use a simple regularization approach that discourages long-range matches. Inspired by weight decay, we add a small multiplicative decay to the flow: $\hat{\mathcal{F}}(\im_1, \im_2) = (1 - \epsilon) \mathcal{F}(\im_1, \im_2)$. This encourages the image prediction to move its prediction closer to its true location in the target. We set $\epsilon = 0.1$ in early stages of training, then set $\epsilon = 0$. % AO: todo

%at the beginning of training to obtain very large flow values, since this is the only way for the flow model to obtain low reconstruction error, leading to solutions that have poor spatial alignment in their output images. % and poor gradient flow. 
%Another failure mode was for the model to predict the identity, and rely on optical flow to bring the prediction closer to ground truth. 


%, to obtain very large flow values, since this is the only plausible. was for the model to predict the identity, and rely on optical flow to bring the prediction closer to ground truth.

%\andrew{I don't think it makes sense to talk about an oracle flow method, does it? if you make a mistake there should always be *some* error, due to occlusions/disocclusion, unless it's a very simple scene}

%One immediate observation we can make is that given an oracle flow method $ \mathcal{F} $, our loss will always be zero, assuming there are no occlusions. Therefore, an optimal strategy to minimizing this loss would be to simply learn the identity function and allow the flow and warping to do all the work. In our initial experiments, even with non-oracle flow, we find that this is in fact the case. \daniel{HERE HERE HERE what does the comment mean?} % AO: not sure if oracle flow is the right framing here

%Upon further inspection, this problem can be solved simply by clipping the flow using



% \begin{equation}
%     \clip(\flow) = \min(\max(\flow, -c), c)
% \end{equation}


%\noindent or it soft variant

To address these issues, we clip the flow before warping:

%slowly introduce optical flow during training, so that the initial stages of training are similar to optimizing only the base loss $\mathcal{L}$, and by limiting the maximum magnitude of the flow. We do this by optimizing
% \begin{equation} \label{eq:clip}
%     \clip(\flow) = c \tanh \left( \frac{\flow}{c} \right),
% \end{equation}
% \noindent where $ c $ is a hyperparameter used to define the clipping threshold. This operation essentially limits the power of the warping function and prevents it from doing all the work. \daniel{Explain in terms of local minima}. Our final loss is then
\begin{equation}
    \mathcal{L}_{warp}(\im, \hat{\im}) = \mathcal{L}(\mathcal{T}(\im; \clip(\mathcal{F}(\im, \hat{\im}))), \hat\im),
\end{equation}
where $\clip$ clips the flow to be in the range $[-c, c]$:
\begin{equation}
\clip(\flow) = c \tanh \left( \frac{\flow}{c} \right).
\end{equation}

This formulation reduces to the base loss $\mathcal{L}$ for $ c = 0 $, leading to a convenient scheduling protocol. In our experiments, we slowly increase $ c $ from 0 to some maximum value determined by the size of the images, but we also found that simply setting a constant value for $ c $ gives similar results. We also note that clipping is commonly used to condition ill-behaved objectives~\cite{arjovsky2017wgan,schulman2017ppo}.

%We note that clipping is commonly used to condition ill-behaved objectives, such as with WGAN~\cite{arjovsky2017wgan} or in PPO~\cite{schulman2017ppo}, and that clipping gracefully reduces to the underlying loss when $ c = 0 $.


\section{Introduction}

Recent years have seen major advances in image synthesis techniques~\cite{isola2016pix2pix, wang2017pix2pixhd, chen2017CRN, park2019spade, karras2018stylegan, brock2018biggan, donahue2019bigbigan}, yet the situations where they can be used remain stubbornly limited. Today's methods can successfully alter a scene's texture, color, or lighting, but struggle to make even tiny changes to {\em position}. Consequently, tasks that require an understanding of motion, such as video prediction, remain challenging open problems.


%Recent years have seen major advances in image synthesis techniques~\cite{isola2016pix2pix, wang2017pix2pixhd, chen2017CRN, park2019spade, karras2018stylegan, brock2018biggan, donahue2019bigbigan}, yet the situations where they can be used remain stubbornly limited. Today's methods can successfully alter a scene's texture, color, or lighting, but struggle to make even tiny changes to {\em position}. As a consequence of these limitations, tasks that require an understanding of motion, such as video forecasting, remain challenging open problems.

%What makes these tasks different is the highly multimodal nature of the prediction problem. Simple ``pixelwise" losses, such as per-pixel $L_2$ distance, assign large penalties to even tiny errors in structure. 
% TODO better transition
One of the key challenges is that image similarity metrics, such as $L_1$ distance between pixels, are highly sensitive to small position errors. %Predicting an object's position %incorrectly under a simple image similarity function %, such as $L_2$ distance, 
%incorrectly under such a loss can result in a catastrophic penalty. 
These losses incentivize models to hedge, producing blurry images that average over the many possible positions an object might occupy.

% probably too long?
Recent work has sought methods that, instead, commit to a single, likely outcome instead of a hedged blur. Perhaps the most common approach, widely used in video prediction, are stochastic models~\cite{kingma2013vae, oord2017vqvae} that learn the full distribution of  outcomes and select a sample. %, rather than estimating the single, low-error outcome. 
Since the full set of possibilities is so large, however, these approaches often struggle fully model them, and nonetheless produce blurry results. Recent work has therefore introduced two other, complementary strategies to obtain crisp prediction results. The first are methods that introduce network layers that force the model to synthesize motion~\cite{zhou2016flow,vondrick2017generating}. Instead of directly synthesizing pixels, these models generate a deformation field, which is then used to warp a source image into a new configuration. However, they require special handling of image content that cannot be easily explained by resampling pixels in an existing image, e.g. via inpainting~\cite{}. They also need complex, special-purpose network architectures that incorporate motion estimation and resampling. Finally, there are methods that aim to obtain {\em spatial invariance} through the use of a perceptual loss. While these loss functions are effective for tiny mistranslations, they break down when errors are more than a few pixels.


%Finally, methods based on perceptual losses obtain a degree of {\em translational invariance} using a learned feature set. 

%cannot be used with standard image synthesis architectures, instead requiring special-purpose architectures that incorporate motion estimation and warping. They also require a way of handling the parts of an image that cannot be explained via motion, such as by inpainting.


%In this paper, we propose, instead, to address this problem by incorporating geometric robustness into.
In this paper, we take inspiration from both of theses approaches, as well as classic work on deformable image matching methods~\cite{barrow1977parametric,huttenlocher1993comparing}, such as Chamfer matching, that geometrically align a template prior to matching an image with it to reduce the cost of positional error.
%, that provide robustness to geometric misalignment within their similarity metrics.
%These methods obtain geometric invariance by aligning a template to a candidate image before estimating their similarity. 
We propose a simple change to off-the-shelf loss functions for image generation. Instead of comparing the two images ``pixelwise", we {\em compare their correspondences}. We put the two images into pixel-to-pixel correspondence using optical flow, then use an off-the-shelf loss function (e.g. $L_1$ distance) to measure the visual similarity between corresponding pixels. 

% (rather than pixels with corresponding $(x, y)$ coordinates). 

% change this depending on what our final set of results are
Despite its simplicity, our proposed ``loss extension" encourages crisp, visually accurate video predictions. Under the resulting loss, every pixel in the ground truth image requires a matching pixel in the predicted image, and vice versa. Blurry, hedged image predictions provide few high-quality matches, and therefore obtain significantly higher loss than images that commit to a single, coherent prediction. Moreover, the loss is still sensitive to position, and encourages models to predict images where objects occupy the right locations. The ground truth image is (except under unusual circumstances) the sole zero-loss solution. Positional errors result in  missing content, such as occluded pixels that are only visible in one image, and in correspondences that have significantly less visual similarity than their matches. 


% AO: rewrite when we get more results!
We apply our method to the task of predicting future frames of egocentric driving videos~\cite{geiger2013IJRR}, a task that requires dealing with uncertainty in motion, position, and 3D structure. %This is a task that requires dealing with a considerable amount of uncertainty. The position and shape of objects in future frames is determined by their motion, their depth, and the egomotion of the camera --- all of which are unknown.  
Since we {\em only} estimate motion as part of the loss function, our method can easily be combined {\em with existing architectures}. This allows us to obtain performance competitive with the state-of-the-art on video prediction, despite using ``off-the-shelf" image translation networks. We also show that our loss can be used in conjunction with existing video prediction models, such as the variational autoencoder-based SVG model~\cite{denton2018stochastic}.

% AO:
The main contributions of our paper are: 1) we propose to handle uncertainty in image prediction tasks by applying loss functions to visual correspondences induced from optical flow; 2) we analyze the resulting loss and show that it has many desirable properties for dealing with uncertainty; 3) we apply our loss to predicting future frames of videos, using a variety of architectures. Our generated videos obtain significantly higher perceptual realism than other methods, as judged by participants in a human study and by automated metrics, and are qualitatively more realistic.

%, which we evalute using human studies and automated metrics. The video frames that our model predicts are sign


%% to the task of predicting future frames of a video.  We show that our model generates videos that are judged by human observers to be significantly more realistic in psychophysical studies than other methods, and that the videos place objects in significantly more accurate positions.




%We also obtain higher accuracy on quantitative metrics that measure the accuracy of the locations of objects in a scene, and on


%We adapt our loss to video prediction. Despite our loss's simplicity, we obtain videos that are rated as significantly more plausible than those of state-of-the-art video future prediction methods.






%One approach for addressing this issue, widely used in video prediction, is to %estimate {\em motion} instead of directly predicting images. Rather than synthesizing images directly, these methods predict an optical flow field, then use it to warp a source image. This gives a generation mechanism that provides a loss that correlates better with perceptual similarity, {\em e.g.}, distance between flow fields

%, and gives a prediction mechanism (e.g., warping) that is incapable of blurring. 

% Two recent approaches have arisen to address this issue for video prediction tasks. The first are methods that explicitly estimate motion~\cite{zhou2016flow,vondrick2017generating,more}. Instead of generating pixels directly, they produce a deformation field, which is then used to warp the input images. These methods, however, require special handling of image content that cannot be easily explained by resampling pixels in an existing image, such as through inpainting~\cite{}, and need special-purpose network architectures that incorporate motion estimation and resampling. Finally, there are methods that aim to obtain {\em spatial invariance} through the use of a perceptual loss. While these loss functions are effective for tiny mistranslations, they break down when errors are more than a few pixels.



%Finally, methods based on perceptual losses obtain a degree of {\em translational invariance} using a learned feature set. 

%cannot be used with standard image synthesis architectures, instead requiring special-purpose architectures that incorporate motion estimation and warping. They also require a way of handling the parts of an image that cannot be explained via motion, such as by inpainting.


%In this paper, we propose, instead, to address this problem by incorporating geometric robustness into.

% from talking to Daniel: consider adding this as third way

 correspondence-based}
 
 % augments an existing loss, or or something
Despite its simplicity, our proposed ``loss extension" leads to significantly crisper and more accurate image predictions. %, in comparison to the underlying loss functions they are based on. 
Under the resulting {\em correspondence-based} loss function, every pixel in a target image requires a high-quality match in the predicted image, and vice versa. The predicted image must also be ``easy to match" for optical flow: not only must every pixel have a , they must satisfy the priors that accompany optical flow models, such as inducing a smooth flow field.  % expanding this.
% For example, the resulting optical flow field must be smooth...
% example
Consequently, blurry (hedged) image predictions tend to obtain higher loss than those that commit to a crisp prediction, since there is no simple transformation that matches them to the target.
% “While at first it may seem that objects may be placed in any location, we show both empirically and theoretically that the optimal solution under our loss has objects in the correct location”
On the other hand, crisp images that place objects in incorrect locations are also heavily penalized, since the loss is sensitive to position. These errors lead to poorer quality matches, as well as missing content, 




---------------------





---------------------


%         \algcomment{\fontsize{7.2pt}{0em}\selectfont \texttt{bmm}: batch matrix multiplication; \texttt{eye}: identity matrix; \texttt{cat}: concatenation.
%         %\vspace{-1.em}
%         }
%         \definecolor{codeblue}{rgb}{0.25,0.5,0.5}
%         \lstset{
%           backgroundcolor=\color{white},
%           basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
%           columns=fullflexible,
%           breaklines=true,
%           captionpos=b,
%           commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
%           keywordstyle=\fontsize{7.2pt}{7.2pt},
%           escapechar=\&% char to escape out of listings and back to LaTeX
%         %  frame=tb,
%         }
% \begin{lstlisting}[language=python]
% # load a minibatch x with B sequences
% for x in loader:  
%   # Split image into patches
%   # B x C x T x H x W -> B x C x T-1 x P x h x w
%   x = unfold(x, (patch_size, patch_size))        
%   x = spatial_jitter(x)
%   # Embed patches (B x C x T x P)
%   v = l2_norm(resnet(x)) 
  
%   # Transitions from t to t+1 (B x T x P x P)
%   A = bmm(v[:,:,:-1], v[:,:,1:]) / temperature
  
%   # Transition similarities for palindrome graph
%   AA = cat((A, A[:,::-1].transpose(-1,-2), 1)
  
%   # Walk
%   At = eye(P)                  &\hspace{21mm}& 
%   for t in range(2*T):                                        &\hspace{49mm}&
%   At = bmm(softmax(dropedge(AA[:,t]),dim=-1), At)
  
%   # Target is the original node (Equation 4)
%   loss = cross_ent_loss(At, labels=[range(P)]*B)     &\hspace{5mm}& 
%   loss.backward()
% \end{lstlisting}
        % \algcomment{\fontsize{7.2pt}{0em}\selectfont \texttt{bmm}: batch matrix multiplication; \texttt{eye}: identity matrix; \texttt{cat}: concatenation.
        % %\vspace{-1.em}
        % }

==> tables/ablations_1.tex <==
\begin{table*}
    \begin{center}
    \resizebox{.9\textwidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule
    & & & \multicolumn{3}{c}{KITTI} & \multicolumn{2}{c}{Caltech} \\
    \cmidrule(lr){4-6} \cmidrule(lr){7-8}
    Setting & Base Loss & Corr. (ours) & SSIM $\uparrow$ & LPIPS $\downarrow$ & 2AFC (\%) $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    \midrule
    \multirow{4}{*}{Fast} 
    & $\mathcal{L}_1 + \mathcal{L}_{p} $ & - & 0.402 $\pm$ 0.02 & 0.309 $\pm$ 0.01 & 33.0 $\pm$ 3.9 & 0.625 $\pm$ 0.03 & 0.207 $\pm$ 0.02 \\ 
    & $\mathcal{L}_1 + \mathcal{L}_{p} $ & \checkmark & {\bf 0.412 $\pm$ 0.02} & {\bf 0.274 $\pm$ 0.01} & 33.0 $\pm$ 3.7 & 0.603 $\pm$ 0.03 & 0.224 $\pm$ 0.02 \\
    \cmidrule(lr){2-8}
    & $\mathcal{L}_1 $ & - & 0.403 $\pm$ 0.02 & 0.444 $\pm$ 0.01 & 32.6 $\pm$ 4.3 & 0.640 $\pm$ 0.03 & 0.303 $\pm$ 0.03 \\ 
    & $\mathcal{L}_1 $ & \checkmark & {\bf 0.439 $\pm$ 0.03} & {\bf 0.405 $\pm$ 0.02} & {\bf 37.4 $\pm$ 4.0} & 0.637 $\pm$ 0.03 & {\bf 0.282 $\pm$ 0.03} \\ 
    \cmidrule{1-8}
    \multirow{4}{*}{Next Frame} 
    & $\mathcal{L}_1 + \mathcal{L}_{p} $ & - & {\bf 0.633 $\pm$ 0.02} & 0.155 $\pm$ 0.01 & 40.1 $\pm$ 2.9 & {\bf 0.788 $\pm$ 0.02} & 0.105 $\pm$ 0.01 \\ 
    & $\mathcal{L}_1 + \mathcal{L}_{p} $ & \checkmark & 0.609 $\pm$ 0.02 & {\bf 0.128 $\pm$ 0.01} & {\bf 47.5 $\pm$ 3.0} & 0.758 $\pm$ 0.02 & 0.112 $\pm$ 0.01 \\ 
    \cmidrule(lr){2-8}
    & $\mathcal{L}_1 $ & - & 0.676 $\pm$ 0.02 & 0.237 $\pm$ 0.01 & 44.5 $\pm$ 3.1 & 0.808 $\pm$ 0.02 & 0.168 $\pm$ 0.02 \\ 
    & $\mathcal{L}_1 $ & \checkmark & 0.681 $\pm$ 0.02 & 0.229 $\pm$ 0.01 & {\bf 47.9 $\pm$ 2.9} & 0.795 $\pm$ 0.02 & {\bf 0.153 $\pm$ 0.01} \\ 
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \vspace{-12pt}

\caption{{\bf Ablations for correspondence-wise losses.} We ablate correspondence-wise losses, showing its efficacy on both the KITTI and Caltech datasets. The third column (``Corr.") indicates the usage of a correspondence-wise loss. 2AFC is the rate at which humans chose the generated video over the true video in a real-or-fake study.
}%Note that the 2AFC metric is bounded by $ 50\% $, which corresponds to a human being unable to differentiate between a real and a generated video. }
\label{tbl:ablations}
\end{table*}


==> tables/ablations_2.tex <==

\begin{table}
    \begin{center}
    \resizebox{.9\linewidth}{!}{
    \begin{tabular}{lcc}
    \toprule
    Ablation & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    \midrule
    None & 0.681 $\pm$ 0.02 & 0.229 $\pm$ 0.01 \\
    Non-symmetric & 0.663 $\pm$ 0.02 & 0.204 $\pm$ 0.01 \\
    No Flow Reg. & 0.670 $\pm$ 0.02 & 0.236 $\pm$ 0.01 \\
    Diff. Thru Flow & 0.675 $\pm$ 0.02 & 0.220 $\pm$ 0.01 \\
    %Classic Flow & 0.673 $\pm$ 0.016 & 0.242 $\pm$ 0.01 \\
    Hom. RAFT & 0.679 $\pm$ 0.02 & 0.238 $\pm$ 0.01 \\
    Farneback Flow & 0.673 $\pm$ 0.02 & 0.242 $\pm$ 0.01 \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    
    \vspace{-13pt}

\caption{{\bf Ablations for several design decisions for our loss}. All ablations use an $L_1$ correspondence-wise loss, trained on KITTI next frame prediction.}
\label{tbl:ablations_extra}
\end{table}


==> tables/ablations_cvpr.tex <==
\begin{table*}
\small
    \begin{center}
    \resizebox{.7\textwidth}{!}{
    \begin{tabular}{ccccccccc}
    %\begin{tabularx}{\linewidth}{ccccccccc}
    \toprule
    & & \multicolumn{3}{c}{KITTI} & \multicolumn{2}{c}{Cityscapes} & \multicolumn{2}{c}{Caltech} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    Base Loss & Corr. & SSIM $\uparrow$ & LPIPS $\downarrow$ & 2AFC (\%) $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    \midrule
    %$L_1$ & - & 0.563 $\pm$ 0.01 & 0.438 $\pm$ 0.01 & 13.52 $\pm$ 1.30 & 0.733 $\pm$ 0.01 & 0.250 $\pm$ 0.01 & 0.820 $\pm$ 0.01 & 0.231 $\pm$ 0.01 \\
    %$L_1$ & \checkmark & {\bf 0.586 $\pm$ 0.01 } & {\bf 0.359 $\pm$ 0.01 } & 14.25 $\pm$ 1.24 & 0.734 $\pm$ 0.02 & {\bf 0.216 $\pm$ 0.01 } & 0.819 $\pm$ 0.01 & 0.198 $\pm$ 0.01 \\
    %\cmidrule(lr){1-9}
    %$L_2^2$ & - & 0.544 $\pm$ 0.01 & 0.499 $\pm$ 0.01 & 13.36 $\pm$ 1.35 & 0.701 $\pm$ 0.01 & 0.330 $\pm$ 0.01 & 0.801 $\pm$ 0.01 & 0.291 $\pm$ 0.01 \\
    %$L_2^2$ & \checkmark & {\bf 0.563 $\pm$ 0.02 } & {\bf 0.403 $\pm$ 0.01 } & 15.16 $\pm$ 1.40 & 0.707 $\pm$ 0.02 & {\bf 0.249 $\pm$ 0.01 } & 0.812 $\pm$ 0.01 & {\bf 0.212 $\pm$ 0.01 } \\
    %\cmidrule(lr){1-9}
    %$L_1+\mathcal{L}_p$ & - & 0.545 $\pm$ 0.01 & 0.213 $\pm$ 0.01 & 14.46 $\pm$ 1.35 & 0.717 $\pm$ 0.02 & 0.139 $\pm$ 0.01 & 0.816 $\pm$ 0.01 & 0.092 $\pm$ 0.00 \\
    %$L_1+\mathcal{L}_p$ & \checkmark & 0.548 $\pm$ 0.01 & {\bf 0.191 $\pm$ 0.01 } & {\bf 20.19 $\pm$ 1.37} & 0.702 $\pm$ 0.02 & 0.141 $\pm$ 0.01 & 0.810 $\pm$ 0.01 & 0.090 $\pm$ 0.00 \\
    $L_1$ & - & 0.563 & 0.438 & 13.52 & {\bf 0.820 } & 0.231 & 0.733 & 0.250 \\
    $L_1$ & \checkmark & {\bf 0.586 } & {\bf 0.359 } & {\bf 14.25} & 0.819 & {\bf 0.198 } & {\bf 0.734 } & {\bf 0.216 } \\
    \cmidrule(lr){1-9}
    $L_2^2$ & - & 0.544 & 0.499 & 13.36 & 0.801 & 0.291 & 0.701 & 0.330 \\
    $L_2^2$ & \checkmark & {\bf 0.563 } & {\bf 0.403 } & {\bf 15.16} & {\bf 0.812 } & {\bf 0.212 } & {\bf 0.707 } & {\bf 0.249 } \\
    \cmidrule(lr){1-9}
    $L_1+\mathcal{L}_p$ & - & 0.545 & 0.213 & 14.46 & {\bf 0.816 } & 0.092 & {\bf 0.717 } & {\bf 0.139 } \\
    $L_1+\mathcal{L}_p$ & \checkmark & {\bf 0.548 } & {\bf 0.191 } & {\bf 20.19} & 0.810 & {\bf 0.090 } & 0.702 & 0.141 \\
    \bottomrule
    \end{tabular}
   }
    \end{center}
    \vspace{-12pt}

\caption{{\bf Ablations for correspondence-wise losses.} We ablate correspondence-wise losses, showing its efficacy on both the KITTI and Caltech datasets. The third column (``Corr.") indicates the usage of a correspondence-wise loss. 2AFC is the rate at which humans chose the generated video over the true video in a real-or-fake study.}
\label{tbl:ablations}
\end{table*}

==> tables/sota_cityscapes.tex <==

\begin{table}
    \begin{center}
    \resizebox{.85\linewidth}{!}{%
    \setlength\tabcolsep{2pt}
    \begin{tabular}{lccccccc}
    \toprule
    %& PN~\cite{lotter2016predictive} & MCnet~\cite{villegas2017decompose} & VF~\cite{liu2017video} & Vid2vid~\cite{wang2018video} & OMP~\cite{wu2020future} & Ours \\
    & Metric & PredNet & MCnet & VoxelFlow & Vid2vid & OMP & Ours \\
    \midrule
    \multirow{2}{*}{Frame 1}
    & SSIM & 0.8403 & 0.8969 & 0.8385 & 0.8816 & 0.8910 & {\bf 0.9056} \\
    & LPIPS & 0.2599 & 0.1888 & 0.1737 & 0.1058 & {\bf 0.0850} & 0.0859 \\
    \bottomrule
    \end{tabular}%
    }
    \end{center}
    
    \vspace{-4mm}
    \caption{{\bf Additional Comparisons.} We present results on next frame prediction on Cityscapes.}
    \label{tbl:sota_cityscapes}
\end{table}
